Discrete Impedance Metasurfaces for 6G Wireless Communications in D-Band

Engineering and optimization of wireless propagation channels will be one of the key elements of future communication technologies. Metasurfaces may offer a wide spectrum of functionalities for passive and tunable reflecting devices, overcoming fundamental limits of commonly used conventional phase-gradient reflectarrays and metasurfaces. In this paper, we develop an efficient way for the design and implementation of metasurfaces with high-efficiency anomalous reflector functionalities. The developed numerical method provides accurate, fast, and simple metasurface designs, taking into account non-local near-field interactions between array elements. The design method is validated by manufacturing and experimental testing of highly efficient anomalous reflectors for the millimetre-wave band.

==> bibliographyBakcup.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{SK_photo.png}}]%
{\bf Sergei~Kosulnikov} Sergei Kosulnikov was born in 1989. He received his B. Sc. and M. Sc. degrees from ITMO University (St. Petersburg, Russia) in 2011 and 2013, respectively. In 2017 he defended a doctoral dissertation in the Department of Electronics and Nanoengineering in Aalto (title is “Wire
media for broadband enhancement of radiation and power transfer”) under the supervision of Prof. Constantin Simovski. In 2018-2021 he worked as a post-doctoral research fellow in the Dynamics of Nanostructures lab. of Tel Aviv University, where his research was targeted on engineering of superscattering and superdirectivity from miniaturized complex EM media structures. He is currently working as a postdoctoral fellow in the group of Prof. S. Tretyakov at the Department of Electronics and Nanoengineering, Aalto University, whereas the research is focused on practical implementation of multichannel metasurfaces for different functionalities.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ST_photo.jpg}}]%
{\bf Sergei A. Tretyakov} (M’92–SM’98–F’08) received the Dipl. Engineer-Physicist, Candidate of Sciences (Ph.D.), and D.Sc. degrees in radiophysics from Saint Petersburg State Technical University, Saint Petersburg, Russia, in 1980, 1987, and 1995, respectively. From 1980 to 2000, he was with the Radiophysics Department, Saint Petersburg State Technical University. He is currently a professor of radio science with the Department of Electronics and Nanoengineering, Aalto University, Aalto, Finland. He has authored or coauthored six research monographs and more than 300  journal papers. His current research interests include electromagnetic field theory, complex media electromagnetics, metamaterials, and microwave engineering. Dr. Tretyakov served as the General Chair for the International Congress Series on Advanced Electromagnetic Materials in Microwaves and Optics (Metamaterials) from 2007 to 2013. He served as the President for the Virtual Institute for Artificial Electromagnetic Materials and Metamaterials (Metamorphose VI). He served as the Chairman for the St. Petersburg IEEE ED/MTT/AP Chapter from 1995 to 1998.
\end{IEEEbiography}

